EraseAnything: Enabling Concept Erasure in Rectified Flow Transformers

Removing unwanted concepts from large-scale text-to-image (T2I) diffusion models while maintaining their overall generative quality remains an open challenge. This difficulty is especially pronounced in emerging paradigms, such as Stable Diffusion (SD) v3 and Flux, which incorporate flow matching and transformer-based architectures. These advancements limit the transferability of existing concept-erasure techniques that were originally designed for the previous T2I paradigm (e.g., SD v1.4). In this work, we introduce EraseAnything, the first method specifically developed to address concept erasure within the latest flow-based T2I framework. We formulate concept erasure as a bi-level optimization problem, employing LoRA-based parameter tuning and an attention map regularizer to selectively suppress undesirable activations. Furthermore, we propose a self-contrastive learning strategy to ensure that removing unwanted concepts does not inadvertently harm performance on unrelated ones. Experimental results demonstrate that EraseAnything successfully fills the research gap left by earlier methods in this new T2I paradigm, achieving state-of-the-art performance across a wide range of concept erasure tasks.

==> sec/acknowledge.tex <==
\section{Acknowledgement}

We extend our heartfelt gratitude to Xingchao Liu from the University of Texas at Austin for his invaluable insights and steadfast support throughout our research journey. His expertise, particularly in the technical intricacies of rectified flow and the nuances of bi-level optimization, has been instrumental in shaping our work. Additionally, we extend our thanks to Shaw, the developer of Eliza (AI16Z)~\footnote{https://github.com/ai16z/eliza}, for creating a tool that has been integral to our research. Our work has utilized Eliza to gather data from the internet and conduct real-world testing.

==> sec/limitations.tex <==
\section{Limitations}

Although "EraseAnything" has demonstrated its formidable ability to erase concepts across various domains, we have identified challenges it faces in certain situations:

\textbf{Extensive Concept Erasure}: When tasked with erasing multiple concepts simultaneously, such as 10 or more concepts (LoRAs), the \textbf{Normalized Sum} strategy, as depicted in \cref{eq:lora_add}, results in a proportional decrease in the impact of each concept's erasure. Consequently, a significant and important avenue for research in this field is to explore efficient methods for combining a large number of LoRAs (more than 100) effectively.


\textbf{Fine-grained Control}: Another issue pertains to the inability to guarantee the strength of the erasure during fine-tuning. This is an uncharted yet intriguing area in the realm of concept erasure, which could provide us with a deeper understanding of the concept formulation. It would also enable more precise control over the erasure process, \textit{e.g.} a slider could be provided to control the intensity during interactive concept erasure.
